Euclidean mirrors and dynamics in network time series

Analyzing changes in network evolution is central to statistical network inference, as underscored by recent challenges of predicting and distinguishing pandemic-induced transformations in organizational and communication networks. We consider a joint network model in which each node has an associated time-varying low-dimensional latent vector of feature data, and connection probabilities are functions of these vectors. Under mild assumptions, the time-varying evolution of the latent vectors exhibits low-dimensional manifold structure under a suitable notion of distance. This distance can be approximated by a measure of separation between the observed networks themselves, and there exist Euclidean representations for underlying network structure, as characterized by this distance, at any given time. These Euclidean representations, called Euclidean mirrors, permit the visualization of network evolution and transform network inference questions such as change-point and anomaly detection into a classical setting. We illustrate our methodology with real and synthetic data, and identify change points corresponding to massive shifts in pandemic policies in a communication network of a large organization.

==> Referee_Report1.tex <==
Review for “Discovering underlying dynamics in time
series of networks”
Abstract
I have positive impression of the paper. However, the paper lacks a lot of needed rigor on
how to interpret latent point process ϕ(·) and the Euclidean mirror ψ(·). As written, it is not
clear how the rates proved in the paper characterize what makes the statistical problem “easy”
or “hard,” how it’s impacted by the time-varying dynamics, and whether or not the difference
in two networks based on the Euclidean mirror is driven primarily by differences in network
sparsity.
The paper “Discovering underlying dynamics in time series of networks” describes a new statistical model for time-varying networks, where the latent position process (a new type of statistical
model) is formulated as the natural extension of latent position graphs to time-varying settings.
The authors 1) formulate a latent process ϕ(·) that has strong mathematical foundations (i.e.,
has meaningful geometry when equipped with the maximum-directional distance k · kMV , ensuring
existence of the Euclidean mirror ψ(·) in Theorem 1, is a manifold in Theorem 2, and continuous
in Theorem 3), and 2) its Euclidean mirror be estimated from data (in Corollary 1). This paper
inherits estimation results for a single latent position graph (specifically the Adjacency Spectral
Embedding), such as from Tang et al. 2017 (see Lemma 4). The authors then analyze a Microsoft
communication network over 24 months, and demonstrate many network diagnostics that stem for
the method.
Overall, I have positive impression of the paper. My major comments regard the interpretation
of the latent point process ϕ(·) and the Euclidean mirror ψ(·). I believe the presentation of the
model is currently incomplete and not yet at the quality needed for a publication in JASA. However, I think all my comments are addressable with enough thoughtful rewriting and additional
text/supplementary materials.
Note: All my page numbers refer to the JASA peer review page number (i.e., page x out of 46).
1 Major remarks
1. Interpretation of the Euclidean mirror: One of the nebulous parts of the paper that
evaded my understanding is what exactly was being captured by ψ(·). I mechanically understand what this is – it’s the Euclidean mirror that best describes the overall temporal shift
1
among n nodes. However, when I look at Figure 4 or consider ψ(·) abstractly, I am not sure
what insight ψ(·) yields.
Here are my current thoughts on what ψ(·) represents. The specific coordinates of ψ(·) are
not too relevant. Rather, the Euclidean distances between two networks (i.e., kψb(s) − ψb(t)k
for time s and t) is a useful way to assess how different two networks are. (As you showed in
Figure 4, you can also deploy this procedure on subnetworks.) The novelty of the paper is not
so much in how to compute kψb(s) − ψb(t)k (this is because thanks to Euclidean realizability,
this calculation is more-or-less simply the sin Θ distance between the spectral embeddings
Xbt and Xbs, see Equation 3). Rather, the novelty is that under a rigorously-defined latent
position process model, there are a wealth of time-varying generalized dot product models
that can explicitly characterize how difficult this estimation task is based on a multitude of
nonparameteric terms (i.e., the Lipschitz and Holder constants).
Note, this is not a criticism of your work. Instead, if the authors agree with my sentiment, I
would like to see the authors make the intended interpretation of ψ(·) and its novelty more
explicit. Most of my comments throughout this review stem from this sentiment.
2. Parameterize of what makes the statistical setting “easy” or “difficult”: To my
understanding, you apply adjacency spectral embedding (ASE) to each individual graph, and
then use the estimated embeddings to compute the sample dMV distances, which is then used
to construct the low-dimensional manifold (for example, running classical multidimensional
scaling (CMDS) on the squared distance matrices Db(2)
ψ
).
My question is: my intuition tells me that a very complex latent process ϕ(·) would make
the estimation task harder. However, it was hard for me to gauge if my intuition was correct,
and how it was reflected in Theorem 6. Specifically, it was unclear to me how large or small
λc(−P ∆D
(2)
ϕ ∆P
>) in Theorem 6 should be. What factors in the network dynamics make
this big or small? Supposedly, this term is closely related to how “wiggly” ϕ(·) is across time,
as I would imagine if the network dynamics is more “non-smooth”, the estimation task gets
“harder.” Is this true?
I mainly ask this because as long as mT is “large enough” (meaning the tail eigenvalues
of Dψ are negligible), I believe all the “hardness” of the estimation task is encapsulated in
λc(−P ∆D
(2)
ϕ ∆P
>). If so, as currently written, it is hard for me to have a grasp of what
exactly λc(−P ∆D
(2)
ϕ ∆P
>) is capturing and what contributes to whether or not its bounded
away from 0.
Concretely: how does the Holder constant α (assumed in Theorem 3 as a concrete example),
Lipschitz constant B, and maximum-distance A defined in Corollary 3 affect λc(−P ∆D
(2)
ϕ ∆P
>)?
If this is not possible to lower-bound for a generic model, can you provide concrete examples
where it can be lower-bounded? (For example, in your Examples 1 and 2 on page 14?)
3. The relevance of time-ordering?: I could be mistaken about the following comment:
It was not clear if the order the T networks A1, . . . , AT impacts the estimation of ψ(·). I
2
do not think so? This is counter-intuitive to me, since certainly the latent position process
(Definition 4) suggests a time-varying dynamic.
As a concrete question: suppose you had the networks analyzed in Section 4, but the networks
were shuffled and no time-information among the 24 networks was provided. I believe you
could still use your procedure to estimate each network evaluated on the Euclidean mirror
ψ(t1), . . . , ψ(tT ), and under some permutation, they would be exactly the same as the ones
you demonstrate in Section 4? If I am correct, is the time-ordering among the 24 networks
purely for interpretation purposes? How does this relate Corollary 3? (It seems like your
estimation procedure is agnostic to the time-ordering of networks, but the rate is dependent
on time-varying parameters? Certainly shuffling the 24 networks would impact the magnitude
of the Lipschitz constant B.) Please clarify this, because although your paper is titled about
“dynamics in time series of networks,” I fear a reader might mistaken the paper to be only
about measuring the differences between a collection of networks (which is not necessarily
ordered by time).
(I suspect this comment is related to the previous comment.)
4. Changes in sparsity?: Does dMV (ϕ(s), ϕ(t)) capture changes in sparsity? For example, if
ϕ(s) = c · ϕ(t) for 0 < c < 1 (i.e., the distribution of latent positions at time s is shrunk
towards 0 compared to that at time t, but the overall network structure remains the same), I
believe dMV (ϕ(s), ϕ(t)) 6= 0. I ask this because most of the motivation in Section 1 suggests
that dMV (ϕ(s), ϕ(t)) is capturing fundamental changes in network structure, not simply a
change in overall edge density.
If I am correct, is it meaningful to “normalize” the graphs beforehand (such as using the
Laplacian)? Even if you do not prove theory for this, it would be immensely helpful for
readers to have practical guidelines (perhaps in the appendix) on how to use your method
and how to appropriately interpret the output.
As a concrete question: during your analysis in Section 4, could I use ψb(·) or its estimated
CMDS or Isomap embedding to distinguish if the connectivity structure (say, in a stochasticblock-model sense) has changed or if the network simply became sparser or denser (uniformly
across all nodes)?
5. More details for Examples 1 and 2: Your model has quite a few moving components (as
it took me a while to understand the latent process ϕ(·) and its Euclidean mirror ψ(·)). Your
Examples 1 and 2 (page 14) were invaluable for my understanding, and I thank the authors
for including them. However, these examples feel somewhat incomplete to me. Here are a
few things I would request the authors to do in the revision. I do not foresee any of these to
be too difficult.
(a) Please include simple simulation examples of either Example 1 or 2 (perhaps in the
appendix). This can be a simple but informative concrete example of γ(t) for a small
number of nodes (say, n = 20), with plots of a few of the graphs along the time series.
Additionally, I believe this example should be simple enough that you can also plot out
3
the population mirror ψ(·) along with the estimated mirror ψb(·) (for example, for c = 3
so you can plot a one-dimensional curve in 3-dimensional space).
(b) I feel Examples 1 and 2 do not intrinsically suggest the more complicated subcommunity behavior in your communication network data in Section 4. I request you to add
an example of a simple time-varying stochastic block model where each node is assigned
to particular community (to be the same for all time points), but the connectivities
between communities can slowly vary over time. For example, you can set K = 3 communities and specify a ϕ(·) such that the between-communities and within-community
probabilities are becoming sparser in certain times or denser in other times. (This would
be informative since I believe your current Examples 1 and 2 can only handle networks
whose mean drift is uniformly becoming denser or sparse across all n nodes, but I could
be mistaken.) This is a pretty simplistic model, but I think it would be incredibly
insightful for readers.
2 Additional remarks
Below are additional remarks of questions I had when reading the paper. I do not expect any
massive new simulation or theory to address these questions as I understand there is already quite
a lot in the paper. Rather, I would like to see a few sentences expanding upon these thoughts in
the main text or supplement, as I believe these additional sentences would be beneficial for readers.
1. I suspect the specific wordings in Section 1 could be improved. You start the section by
discussing the green and blue subcommunitites in Figure 1 and discuss about how to “gauge
differences across scales, from nodes to sub-networks to the entire network itself,” but your
theory is for the differences for the entire network. Do you have theory for sub-networks
or for individual nodes? Could existing entrywise bounds (i.e., k · k2→∞ norm) be used to
specifically ask questions about individual nodes? I do not expect you to proof these theorems
if they are outside the scope of this current paper. Rather, I would like to see a more clear
narrative in Section 1 since I had the wrong impression of what your theory was intended to
show while I was reading Section 3.
2. In terms of writing, for how central Figure 3 is to your paper (page 19), it receives very
little exposition in Section 3. Please adjust the writing to make the importance/novelty of
Figure 3 more apparent to readers. I ask this mainly because in the Discussion, you highlight
the importance of Figure 3, writing, “The perspective described in Figure 3, which connects
distance metrics for generative processes of networks to their estimates, and in turn translates
manifold geometry into Euclidean geometry, is an important theoretical contribution to time
series analysis for networks.”
3. I didn’t quite understand how to read the Isomap embedding plot in Figure 4. This isn’t the
Euclidean mirror being plotted, so how I should interpret the y-axis? Should I be focusing
4
on relative differences in the y-axis between consecutive points, and the relative difference
captures broad differences in the networks across time?
3 Minor remarks
Below are minor remarks I hope the authors will find useful in improve the clarity of the paper.
1. On page 7, you define X1, . . . , Xn ∈ R
d as specific realization of d-dimensional latent positions
for n nodes. However, on page 9, I believe you define Xt = X(t, ·), which is the distribution of latent positions in d-dimensions. It would be helpful to the reader to either clarify
this somewhere in Section 2 or to use superscripts to contrast time from node indexing (for
example, X(t)
).
2. When you first introduce your data in page 2, it was not clear to me what each node represents.
I presume it’s an individual (i.e., an employee of a Microsoft)? Please include a bit more
description in your main text – what does a node and edge represent?
3. Please include a bit more description on why a reader would intuitively think the green
community had a constant drift while the blue had a shock from Figure 1. (I understand this
was more apparent from Figure 4, but when I first read the paper, I was not sure what I was
supposed to see when I looked at Figure 1 in isolation.) Perhaps having 4 networks instead
of only 2 would make it more apparent what a “sudden shock” looks like?
4. Please improve the explanation of Figure 2 in Section 1. I did not quite understand Figure 2
until I got to page 21.
5. Please be more explicit about the model (bottom of page 8). Specifically, for sake of clarity, please write the Bernoulli sampling of each edge conditional of X(t, ωi) and X(t, ωj ).
Supposedly the model for random dot product graphs would like something like
At,ij ∼ Bernoulli
X(t, ωi)
>X(t, ωj )

.
(This is because Definition 1 might seem opaque to a reader not already familiar with latent
position random graphs.)
6. When reading the paper, it was not super clear why k · kMV norm was specifically used
(definition 3, page 9). After reading the paper a few times and looking into the proofs,
my conclusion was that k · kMV is the appropriate norm since it is the population analogy
of Procrustes alignment. Is my understanding correct? I comment on this because when I
read Section 2 for the first time, I did not see much motivation on why exactly this specific
norm was used. If my understanding is correct, please include this (for example, right above
Remark 2).

7. Please clarify the norms. My understanding is that k · k referred to the Euclidean norm for
vectors (see Definition 6), while k · k2 referred to the spectral norm for matrices, and k · kF
the Frobenius norm for matrices. If I am correct, please write this explicitly.
8. I was a bit unsure about nonbacktracking condition in Definition 4 (page 10). To my understanding ϕ(t) is a d-dimensional probability distribution on L
2
(Ω). Does your nonbacktracking condition simply mean this distribution can not exactly be the same at any two
times unless it has remained the same for a period of time? Specifically, when I look at your
“deterministic-drift plus noise” model near page 13, does this mean the deterministic drift γ(t)
can backtrack as long as the variance of Mt
is strictly monotonically increasing/decreasing
with time t?
9. I suspect there is formatting error in Definition 6. Also, please be concrete on how dMV (ϕ(t), ϕ(t
0
))
is defined prior to Definition 6.
10. In Example 1 (page 14), what is the importance of realize that I(t) is not an Ft-martingale?
It was not immediately obvious to me. Also, for sake of completeness, please bound the
Lipschitz constant B and maximum-distance A for both Examples 1 and 2 so readers have
an easier time understanding Corollary 3. (You can state these bounds when you describe
Corollary 3, or include them in the supplement if you feel it is too distracting in the main
text.) Additionally, it would be good to clarify that c = 1 in both examples.
11. While it was clear to me what the estimation procedure (starting page 15) is, I do not think
it would be immediately obvious to a new reader. Please make the procedure more formal,
perhaps with a pseudocode, starting from the observed adjacency matrices A1, . . . , AT and
ending with the estimated Euclidean mirror ψb(·) (as shown in Corollary 2). You can include
this in the Supplement if you find it too distracting in the main text.
12. Please state that Equation 3 is related to the sin Θ distance, so readers can related your
distance to the broader literature.
13. Please remind the reader what vi and vj are in Equation 4 (page 16). Are you still assuming
the model in Examples 1 and 2 here? I understood vi and vj as simply ψ(ti) and ψ(tj ), but
I could be mistaken.
14. For the sake of clarity, I would appreciate if Corollary 3 had the simplest possible version of
estimating ψ(·) (like how you write in Corollary 2). In particular, it would help to have all
networks be equally-spaced in time to remove all the ∆ti terms. I only ask this since it took
me a while to see the “most important factors” that dictate how fast the rate of convergence
is in a simplistic setting.
15. I suspect there is a typo in Corollary 1 (page 17), where I believe it should read kDb(2)
ϕ −D
(2)
ψb
kF ?
16. Is sigimage a term commonly used in ISOMAP embeddings? I was not familiar with this
term, despite its frequent usage. Are you coining this term?
6
17. Overall, please include the specific formulas for the downstream analyses performed in Section
4. For example, 1) in Figure 5 (page 23), it was not clear what the “mean embedding” is. Is
the mean of the each network’s ISOMAP embedding, or the ISOMAP of the averaged latent
embeddings? (I imagine it is the latter, but I am not sure.) 2) I was not sure how “standard
deviation” was computed (but I assume this the standard deviation of each node across the
5 embeddings, averaged over all nodes)? 3) How was the “linear regression” performed?
These specific equations I am asking for can be put in the appendix.
18. Please improve Figure 6 (page 24), as currently, it is hard to see what you’re trying to show.
Perhaps the bootstrap curves can be represented as bands, and there are can be different
panels for different ns values?
19. In the Discussion (page 27), you never really mention the specific terms “GEE” or “Procrustesaligned” through the paper, despite these terms have a spotlight in the Discussion. Please
incorporate these terms more throughout the paper. (To be frank, I’m not entirely sure what
GEE is, so I would appreciate a brief description in the appendix.)
20. For clarity, please put the original sigimage values onto Figure 7 (supposedly, these are the
values shown in Figure 5 (left)?) It would be helpful to see the original sigimage values plotted
directly ontop of the 100 replicates. You might mark the original sigimage as black dots for
visual clarity.
21. On page 41, I personally did not find the cited result for Lemma 4 in Tang et al. (2017)
or Athreya et al. (2022). To my understanding, you are invoking one of the lemmas after
a supposedly-simple reparameterization? In any case, please make this more clear (perhaps
citing the specific result used in either of the two papers, and providing the appropriate
reparameterization steps if used). This would help new readers understand the result.
22. There is a minor typo in page 42 (i.e., missing space in “challenge, however,is the maximization”).
23. In the appendix, please provide more plots and summary statistics of the communication
network data. It seems like you have 24 different networks, each with the same set of 33
communities. Please plot a handful (for example, 6 of them, aside from the 2 already shown
in Figure 1), highlight a few (for example, 5) of the 33 communities. Also, please provide
information on the overall sparsity of the 24 networks and other useful common networkstatistics to help the reader understand your data (for example, number of partitions, average
centrality, etc.) This can be any statistics you think is useful, because as currently written,
it is hard for the reader to appreciate the trends you are showing in Section 4.
24. Please include the proof of Corollary 1 for completeness.
